A Framework for Blockchain Interoperability and Runtime Selection

The suitability of a particular blockchain for a given use case depends mainly on the blockchain's functional and non-functional properties. Such properties may vary over time, and thus, a selected blockchain may become unsuitable for a given use case. This uncertainty may hinder the widespread adoption of blockchain technologies in general. To mitigate the impact of volatile blockchain properties, we propose a framework that monitors several blockchains, allows the user to define functional and non-functional requirements, determines the most appropriate blockchain, and enables the switchover to that chain at runtime. Our evaluation using a reference implementation shows that switching to another blockchain can save cost and enable users to benefit from better performance and a higher level of trust.

==> sections/05_discussion.tex <==
%\section{Discussion}
%\label{sec:discussion}

